Enhancing Box and Block Test with Computer Vision for Post-Stroke Upper Extremity Motor Evaluation

Standard clinical assessments of upper-extremity motor function after stroke either rely on ordinal scoring, which lacks sensitivity, or time-based task metrics, which do not capture movement quality. In this work, we present a computer vision-based framework for analysis of upper-extremity movement during the Box and Block Test (BBT) through world-aligned joint angles of fingers, arm, and trunk without depth sensors or calibration objects. We apply this framework to a dataset of 136 BBT recordings collected from 48 healthy individuals and 7 individuals post stroke. Using unsupervised dimensionality reduction of joint-angle features, we analyze movement patterns without relying on expert clinical labels. The resulting embeddings show separation between healthy movement patterns and stroke-related movement deviations. Importantly, some patients with the same BBT scores can be separated with different postural patterns. These results show that world-aligned joint angles can capture meaningful information of upper-extremity functions beyond standard time-based BBT scores, with no effort from the clinician other than monocular video recordings of the patient using a phone or camera. This work highlights the potential of a camera-based, calibration-free framework to measure movement quality in clinical assessments without changing the widely adopted clinical routine.

==> limitations.tex <==
Although we prove a way of separating stroke patients from healthy individuals just through 3D joint angle analysis with state-of-the-art computer vision methods, there are several limitations that should be considered when interpreting the results. First, the number of stroke patients is limited, with data collected from seven individuals across twenty sessions. This limits the generalizability of the observed movement patterns across different stroke severities or symptoms of stroke. Second, all joint angles are estimated from monocular RGB video, which is inherently subject to depth ambiguity, self-occlusion, and reduced accuracy during complex hand-object interactions. Finally, the analysis is restricted to a single standardized task, the Box and Block Test, performed from a fixed camera viewpoint under controlled conditions. The framework has not been evaluated on other rehabilitation tasks.

==> tables/table2.tex <==
\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{lcccc}
\toprule
Method & PA-MPJPE & PA-MPVPE & F@5 & F@15 \\
\midrule
WiLoR \cite{potamias2024wilor} & \textbf{5.5} & \textbf{5.1} & \textbf{0.825} & \textbf{0.993} \\
SAM 3D Body \cite{yang2025sam3dbody} & \textbf{5.5} & 6.2 & 0.737 & 0.988 \\
\bottomrule
\end{tabular}
\caption{Comparison of hand pose estimation methods on FreiHAND \cite{Freihand2019} where the best results are highlighted in bold.}
\label{tab:hand_pose}
\vspace{-1.5em}
\end{table}
